The power and Arnoldi methods in an algebra of circulants

Circulant matrices play a central role in a recently proposed formulation of three-way data computations. In this setting, a three-way table corresponds to a matrix where each "scalar" is a vector of parameters defining a circulant. This interpretation provides many generalizations of results from matrix or vector-space algebra. We derive the power and Arnoldi methods in this algebra. In the course of our derivation, we define inner products, norms, and other notions. These extensions are straightforward in an algebraic sense, but the implications are dramatically different from the standard matrix case. For example, a matrix of circulants has a polynomial number of eigenvalues in its dimension; although, these can all be represented by a carefully chosen canonical set of eigenvalues and vectors. These results and algorithms are closely related to standard decoupling techniques on block-circulant matrices using the fast Fourier transform.

==> ggv2010-old.tex <==
%In this paper, we interpret three-way data as a matrix
%over a ring of circulant matrices.  That is, given
%an element in $\RR^{m \times n \times k}$, we view
%it as a $m \times n$ matrix over a ring of $k$-parameter
%``scalars.''  Such an interpretation was recently
%proposed by \citet{kilmer2008-circ-tensor-svd}.  
%Their idea was to define a coherent system 
%in which a three-way tensor acts on a matrix and
%produces a matrix, just 
%as a matrix acts on a vector and produces a vector.
%From these definitions, they propose an algorithm
%to decompose a tensor in a manner similar
%to the singular value decomposition, and propose
%a QR-like decomposition.   
%\citet{braman201x-tensor-eigenvalues} then showed 
%these tensor operations corresponds to linear
%transformations in free module --
%a generalization of a vector space over a ring instead
%of a field.  What this statement implies is that \emph{many}
%of the properties and decompositions of matrices over $\RR$ will hold
%for these matrices over circulants, albeit with 
%some key differences.
%
%Our ultimate goal is to introduce and state
%\emph{iterative} algorithms in this free module.  
%
%These algorithms only access the tensor by 
%way of tensor-matrix operations; although, we find it
%more convenient to think of the extension as a standard
%matrix-vector product over $k$ parameter scalars.  
%Over the course of this paper, we build towards this goal
%by defining new operations, such as conjugation, in the ring of 
%circulant matrices and  we expand on the circulant 
%matrix algebra by defining an inner-product.  

% this view of tensor data contradicts with
% many others.  

% important points to discuss: tensors are not really
% tensors; 


% where 
%
%There are many ways to interpret a three-way table.  By that, 
%we mean: given an element of $\RR^{m \times n \times k}$,
%what it it?  In statistics, such an item is known as a 
%data-cube.  It isIn multilinear algebra, elements in $\RR^{m \times n \times k}$
%represent a multilinear change of basis operation -- just like an
%element of $\RR^{m \times n}$ represents a change of basis
%for a vector space.  
%
%Furthermore, multiway data is common in multivariate polynomial
%approximation.  There, the coefficients 
%
%\begin{verbatim}
%How to interpret 3-way data
%  -- As a table : statistics
%  -- As a multilinear operator : Lek, Tammy
%  -- As a ``matrix'' over k-parameter ``scalars'' : Bramen, etc.
%Our contributions
% -- Fleshing out the circulant algebra; we add functions,
%    conjugates, magnitudes, and other standard constructions
% -- Adding a norm to the circulant free module
% -- Investigating historical developments in the circulant algebra
% -- Define and investigate iterative algorithms in the circulant algebra
% -- Relationship between derivations in the Circulant Algebra and
%    standard relationships on block circulant matrices
%    (e.g. Arnoldi is more economical when you do the 
%     circulant algebra version in comparison with the standard 
%     implementation)
% -- A user-friendly Matlab code for working with the circulant algebra
% -- Numerical examples of our approach and algorithms
%\end{verbatim}
%
%We use the term hypermatrix and tensor interchangably to refer to an 
%element of $\RR^{m \times n \times k}$.  We can interpret this tensor as a multi-index
%array of data or as a multi-linear transform.  For the former, defining
%a Krylov space is problematic because there is no clear analog of the ``matrix-vector''
%product.  For the later, the operations are well defined, but they
%make an Arnoldi algorithm extremely complicated \cite{savas2009-krylov}.
%
%%Under another view of a tensor, the answer is yes.
%In another view of a tensor, we can concert it as a matrix where 
%each element is from an algebraic structure parameterized by $k$
%real values.  
%Recent work on tensor factorizations showed that viewing tensors
%as matrices on the circulant algebra provides simple extensions
%of the SVD, QR, and Schur factorizations to three dimensional datasets 
%\cite{kilmer2008-circ-tensor-svd}.
%That is, if we identify an $\RR^{m \times n \times k}$ tensor 
%with a matrix defined on a circulant
%algebra (where each ``scalar'' is defined by $k$ numbers), then applying
%a matrix algorithm produces a useful tensor result.  

% Look at tensors as matrices of circulants.
% Corresponds to operations recently proposed by Kilmer, and identified
% as a free-module by Braman.
% 
% Tensors, or matrices over a ring?  We adopt the latter view; we find it
% a convenient representation for our discussion.
% 
% We view tensors, three-way data, and three-way arrays as interchangeable
% terms to describe elements in $\RR^{m \times n \times k}$. 
% For some problems in statistics -- , the goal is only an analysis
% of the multi-way table \cite{barnard1936-contingency-tables,lancaster1951-contingency}.  
% This view is common in statistics and it is 
% 
% Our goal: iterative algorithms.
% 
% 
% 
% Summary of contributions
% 
% 
% Our setting, (what we look at)
% a key property of our analysis, (why we look at it this way)
% a high level view of our analysis compared to others (what else are people looking at)
% (here is the transition into our material)
% our goal is iterative algorithms
% this requires us to flesh out the free module
% we
% 
% Organization of the paper:
% Notation to distinguish matrices over $\RR$ from matrices over $\KK$, general
% notation standards.
% 
% (Alternative, reference sections as we explain what we need to change
% with the power method; 
%

%This philosophy has implications for our definition and notations, which
%differ from \citet{kilmer2008-circ-tensor-svd} and 
%\citet{braman201x-tensor-eigenvalues}.  These differences are
%aesthetic, we use identical operations.  
%For example, the tensor-matrix product defined by
%\citet{kilmer2008-circ-tensor-svd} becomes a matrix-vector
%product in our view.  

% We continue in the next section by explaining the notation
% conventions in the paper. Our exposition continues by 
% briefly reviewing a few key properties of circulant 
% matrices, stating the ring of circulant matrices, 
% and the free module.  For the free module, we review
% the operations between matrices,
% vectors, and scalars.  We relate these to the definitions
% of tensor operations from \citet{kilmer2008-circ-tensor-svd}.

%his property also yields a set of conditions for a
%set of complex-valued eigenvalues to correspond with a real-valued
%circulant matrix.  

% 
% \begin{center}
% \begin{tabular}{ccl}
%   $\calpha + \cbeta$ & is addition & $\calpha + \cbeta =_k \tvec(\calpha) +  \tvec(\cbeta)$ \\
% $\calpha \circ \cbeta$ & is multiplication & $\calpha \circ \cbeta =_k \tcirc(\alpha) \tvec(\cbeta)$ \\
%   $\cone$ & is the identity & $\cone =_k \bmat{1 & 0 & \ldots & 0}$ \\
% $\calpha^{-1}$ & is the inverse & $\calpha^{-1} =_k \tcirc(\calpha)^{-1} \ve_1$ \\
%   $f(\calpha)$ & is an arbitrary funciton & $f(\calpha) =_k f(\tcirc(\calpha))$ \\
% \end{tabular}
% \end{center}

% 
% \subsection{Summary of basic properties}
% 
% \begin{itemize}
%  \item commutativity
%  \item identity element
%  \item inverse
%  \item function
%  \item pseudo-inverse 
%  \item circ
%  \item vec 
%  \item matrix ``inplace'' notation 
%  $\bmat{ \sbmat{A_{1,1}^{1} & \ldots & A_{1,1}^{k}} & \ldots & \sbmat{A_{1,n}^{1} & \ldots & A_{1,n}^{k}} \\
%          \vdots & \ddots & \vdots \\
%          \sbmat{A_{m,1}^{1} & \ldots & A_{m,1}^{k}} & \ldots & \sbmat{A_{m,n}^{1} & \ldots & A_{m,n}^{k}} } $
% 
% \end{itemize}

% In this section, we review properties of this algebra.
% Let $\alpha, \beta \in \KK_k$.  
% \begin{quote}
% \begin{tabularx}{\linewidth}{rX}
%  identity & $\imath = \bmat{ 1 & 0 & \ldots 0 }$ \\ \addlinespace
%  commutativity & $\alpha \odot \beta = \beta \odot \alpha$ \\
%  inversion & $\alpha^{-1} \equiv \tcirc(\alpha)^{-1} \cdot \ve_1$\\
% \end{tabularx}
% \end{quote}
% 
% The identity easily follows from the relationship with 
% circulant matrix algebra where it becomes the identity matrix.
% Commutativity also follows from commutativity of circulant matrices.
% \[ \alpha \odot \beta = \beta \odot \alpha \Leftrightarrow 
%   \tcirc(\alpha) \tcirc(\beta) \ve_1 = \tcirc(\beta) \tcirc(\alpha) \ve_1. \]
% The inverse element is also easy to see via the definition of multiplication:
% $\va \circ \vb = \tcirc(\va) \vb$.
% 
% Not all elements have an inverse.  Note that any element $\va \in \KK_k$
% with $\sum_i a_i = 0$ does not have an inverse.  \todo{mention that this
% property follows from discussions in the previous section on circulant.}
% 
% For other functions, such as absolute values and square roots, we use
% definitions based on the functions of matrices.  Let $f(x)$ be a scalar
% function.  The equivalent function in the circulant algebra is 
% $f(\tcirc(\alpha)) \ve_1$, where we use the standard definition
% of $f$ applied to a matrix.
% \todo{ explain that this definition is equivalent to applying
% the function to the eigenvalues.}


%While this definition is a natural extension of the other definitions
%in this algebra, the following theorem provides a more natural 
%interpretation of conjugation.
%\begin{theorem}
% Let $\calpha \in \KK_k$ where $\tvec(\calpha) = \bmat{a_1 & a_2 & \ldots & a_k}^T$.
% Then 
% \[ \conj{\calpha} = \fftm^2 \tvec(\va) \]
% and equivalently
% \[ \conj{\calpha} = \bmat{a_1 & a_k & a_{k-1} & \ldots & a_2}. \]
%\end{theorem}
%\begin{proof}
%  First, note that 
%  \[                    
%     \fftm^2 = \bmat{1 & 0 & \ldots & 0 & 0 \\
%                     0 & 0 & \ldots & 0 & 1 \\
%                     \vdots & \vdots & \iddots & \iddots & \vdots \\
%                     0 & 0 & \iddots & 0 & 0 \\
%                     0 & 1 & \ldots & 0 & 0 }.
%  \]
%  This observation follows from well known properties of the Fourier matrix.
%  Using this result shows the equivalence between the two 
%  formulations in the thoerem.  What remains is
%  to establish $\conj{\calpha} = \fftm^2 \tvec(\calpha)$.  
%  Note that $\fftm^{-1} = \ifftm = \conj{\fftm}$ because the Fourier matrix
%  is complex symmetric ($\fftm^T = \fftm$) and unitary ($\fftm \ifftm = \eye$).
%  By definition, then
%  \[ \conj{\calpha} = \ifftm ( \conj{\fftm \tvec(\calpha) } ) = \ifftm \conj{\fftm} \tvec(\calpha) = \fftm^2 \tvec(\calpha) \]
%  because $\tvec(\calpha)$ is entirely real and $\ifftm^2 = \fftm^2$. 
%\end{proof}

Before proceeding to show the remainder of the properties for the conjugate,
let us briefly show one small lemma.
\begin{lemma}
 $\fftm^2 \tcirc(\calpha) = \tcirc(\fftm^2 \tvec(\calpha)) \fftm^2$
\end{lemma}
\begin{proof}
 First, note that $\tcirc(\fftm^2 \va) = \tcirc(\va)^T$.  Let 
 $\tcirc(\va) = \fftm \mLambda \ifftm$.  Then 
 $\fftm^2 \fftm \mLambda \ifftm = \ifftm \mLambda \ifftm = \fftm \mLambda^\ast \fftm$,
 where we used $\fftm^3 = \ifftm$, $\fftm^T = \fftm$, and the fact that the
 left hand side is a real matrix, so we can take the complex conjugate of everything.  
 Using the eigenvectors of $\tcirc(\calpha)$ to expand the transpose in the right 
 hand side produces $\fftm \mLambda^\ast \ifftm \fftm^2 = \fftm \mLambda^\ast \fftm$.
\end{proof}

